Search for the doubly heavy $\mathit{\Xi}_{bc}^{0}$ baryon via decays to $D^0pK^-$

A search for the doubly heavy $\mathit{\Xi}_{bc}^{0}$ baryon using its decay to the $D^0pK^-$ final state is performed using proton-proton collision data at a centre-of-mass energy of 13 TeV collected by the LHCb experiment between 2016 and 2018, corresponding to an integrated luminosity of 5.4 $\mathrm{fb}^{-1}$. No significant signal is found in the invariant mass range from 6.7 to 7.2 $\mathrm{GeV}/c^2$. Upper limits are set at $95\%$ credibility level on the ratio of the $\mathit{\Xi}_{bc}^{0}$ production cross-section times its branching fraction to $D^0pK^-$ relative to that of the $\mathit{\Lambda}_{b}^{0} \to D^0pK^-$ decay. The limits are set as a function of the $\mathit{\Xi}_{bc}^{0}$ mass and lifetime hypotheses, in the rapidity range from 2.0 to 4.5 and in the transverse momentum region from 5 to 25 $\mathrm{GeV}/c$. Upper limits range from $1.7\times10^{-2}$ to $3.0\times10^{-1}$ for the considered $\mathit{\Xi}_{bc}^{0}$ mass and lifetime hypotheses.

==> LHCb_Authorship_12-May-2020_arXiv.tex <==
LHCb collaboration:
R. Aaij,
C. Abell{\'a}n Beteta,
T. Ackernley,
B. Adeva,
M. Adinolfi,
H. Afsharnia,
C.A. Aidala,
S. Aiola,
Z. Ajaltouni,
S. Akar,
J. Albrecht,
F. Alessio,
M. Alexander,
A. Alfonso Albero,
Z. Aliouche,
G. Alkhazov,
P. Alvarez Cartelle,
A.A. Alves Jr,
S. Amato,
Y. Amhis,
L. An,
L. Anderlini,
G. Andreassi,
A. Andreianov,
M. Andreotti,
F. Archilli,
A. Artamonov,
M. Artuso,
K. Arzymatov,
E. Aslanides,
M. Atzeni,
B. Audurier,
S. Bachmann,
M. Bachmayer,
J.J. Back,
S. Baker,
P. Baladron Rodriguez,
V. Balagura,
W. Baldini,
J. Baptista Leite,
R.J. Barlow,
S. Barsuk,
W. Barter,
M. Bartolini,
F. Baryshnikov,
J.M. Basels,
G. Bassi,
V. Batozskaya,
B. Batsukh,
A. Battig,
A. Bay,
M. Becker,
F. Bedeschi,
I. Bediaga,
A. Beiter,
V. Belavin,
S. Belin,
V. Bellee,
K. Belous,
I. Belov,
I. Belyaev,
G. Bencivenni,
E. Ben-Haim,
A. Berezhnoy,
R. Bernet,
D. Berninghoff,
H.C. Bernstein,
C. Bertella,
E. Bertholet,
A. Bertolin,
C. Betancourt,
F. Betti,
M.O. Bettler,
Ia. Bezshyiko,
S. Bhasin,
J. Bhom,
L. Bian,
M.S. Bieker,
S. Bifani,
P. Billoir,
M. Birch,
F.C.R. Bishop,
A. Bizzeti,
M. Bj{\o}rn,
M.P. Blago,
T. Blake,
F. Blanc,
S. Blusk,
D. Bobulska,
V. Bocci,
J.A. Boelhauve,
O. Boente Garcia,
T. Boettcher,
A. Boldyrev,
A. Bondar,
N. Bondar,
S. Borghi,
M. Borisyak,
M. Borsato,
J.T. Borsuk,
S.A. Bouchiba,
T.J.V. Bowcock,
A. Boyer,
C. Bozzi,
M.J. Bradley,
S. Braun,
A. Brea Rodriguez,
M. Brodski,
J. Brodzicka,
A. Brossa Gonzalo,
D. Brundu,
A. Buonaura,
C. Burr,
A. Bursche,
A. Butkevich,
J.S. Butter,
J. Buytaert,
W. Byczynski,
S. Cadeddu,
H. Cai,
R. Calabrese,
L. Calefice,
L. Calero Diaz,
S. Cali,
R. Calladine,
M. Calvi,
M. Calvo Gomez,
P. Camargo Magalhaes,
A. Camboni,
P. Campana,
D.H. Campora Perez,
A.F. Campoverde Quezada,
S. Capelli,
L. Capriotti,
A. Carbone,
G. Carboni,
R. Cardinale,
A. Cardini,
I. Carli,
P. Carniti,
K. Carvalho Akiba,
A. Casais Vidal,
G. Casse,
M. Cattaneo,
G. Cavallero,
S. Celani,
R. Cenci,
J. Cerasoli,
A.J. Chadwick,
M.G. Chapman,
M. Charles,
Ph. Charpentier,
G. Chatzikonstantinidis,
C.A. Chavez Barajas,
M. Chefdeville,
C. Chen,
S. Chen,
A. Chernov,
S.-G. Chitic,
V. Chobanova,
S. Cholak,
M. Chrzaszcz,
A. Chubykin,
V. Chulikov,
P. Ciambrone,
M.F. Cicala,
X. Cid Vidal,
G. Ciezarek,
P.E.L. Clarke,
M. Clemencic,
H.V. Cliff,
J. Closier,
J.L. Cobbledick,
V. Coco,
J.A.B. Coelho,
J. Cogan,
E. Cogneras,
L. Cojocariu,
P. Collins,
T. Colombo,
L. Congedo,
A. Contu,
N. Cooke,
G. Coombs,
S. Coquereau,
G. Corti,
C.M. Costa Sobral,
B. Couturier,
D.C. Craik,
J. Crkovsk\'{a},
M. Cruz Torres,
R. Currie,
C.L. Da Silva,
E. Dall'Occo,
J. Dalseno,
C. D'Ambrosio,
A. Danilina,
P. d'Argent,
A. Davis,
O. De Aguiar Francisco,
K. De Bruyn,
S. De Capua,
M. De Cian,
J.M. De Miranda,
L. De Paula,
M. De Serio,
D. De Simone,
P. De Simone,
J.A. de Vries,
C.T. Dean,
W. Dean,
D. Decamp,
L. Del Buono,
B. Delaney,
H.-P. Dembinski,
A. Dendek,
V. Denysenko,
D. Derkach,
O. Deschamps,
F. Desse,
F. Dettori,
B. Dey,
P. Di Nezza,
S. Didenko,
L. Dieste Maronas,
H. Dijkstra,
V. Dobishuk,
A.M. Donohoe,
F. Dordei,
M. Dorigo,
A.C. dos Reis,
L. Douglas,
A. Dovbnya,
A.G. Downes,
K. Dreimanis,
M.W. Dudek,
L. Dufour,
V. Duk,
P. Durante,
J.M. Durham,
D. Dutta,
M. Dziewiecki,
A. Dziurda,
A. Dzyuba,
S. Easo,
U. Egede,
V. Egorychev,
S. Eidelman,
S. Eisenhardt,
S. Ek-In,
L. Eklund,
S. Ely,
A. Ene,
E. Epple,
S. Escher,
J. Eschle,
S. Esen,
T. Evans,
A. Falabella,
J. Fan,
Y. Fan,
B. Fang,
N. Farley,
S. Farry,
D. Fazzini,
P. Fedin,
M. F{\'e}o,
P. Fernandez Declara,
A. Fernandez Prieto,
J.M. Fernandez-tenllado Arribas,
F. Ferrari,
L. Ferreira Lopes,
F. Ferreira Rodrigues,
S. Ferreres Sole,
M. Ferrillo,
M. Ferro-Luzzi,
S. Filippov,
R.A. Fini,
M. Fiorini,
M. Firlej,
K.M. Fischer,
C. Fitzpatrick,
T. Fiutowski,
F. Fleuret,
M. Fontana,
F. Fontanelli,
R. Forty,
V. Franco Lima,
M. Franco Sevilla,
M. Frank,
E. Franzoso,
G. Frau,
C. Frei,
D.A. Friday,
J. Fu,
Q. Fuehring,
W. Funk,
E. Gabriel,
T. Gaintseva,
A. Gallas Torreira,
D. Galli,
S. Gallorini,
S. Gambetta,
Y. Gan,
M. Gandelman,
P. Gandini,
Y. Gao,
M. Garau,
L.M. Garcia Martin,
P. Garcia Moreno,
J. Garc{\'\i}a Pardi{\~n}as,
B. Garcia Plana,
F.A. Garcia Rosales,
L. Garrido,
D. Gascon,
C. Gaspar,
R.E. Geertsema,
D. Gerick,
L.L. Gerken,
E. Gersabeck,
M. Gersabeck,
T. Gershon,
D. Gerstel,
Ph. Ghez,
V. Gibson,
M. Giovannetti,
A. Giovent{\`u},
P. Gironella Gironell,
L. Giubega,
C. Giugliano,
K. Gizdov,
E.L. Gkougkousis,
V.V. Gligorov,
C. G{\"o}bel,
E. Golobardes,
D. Golubkov,
A. Golutvin,
A. Gomes,
S. Gomez Fernandez,
F. Goncalves Abrantes,
M. Goncerz,
G. Gong,
P. Gorbounov,
I.V. Gorelov,
C. Gotti,
E. Govorkova,
J.P. Grabowski,
R. Graciani Diaz,
T. Grammatico,
L.A. Granado Cardoso,
E. Graug{\'e}s,
E. Graverini,
G. Graziani,
A. Grecu,
L.M. Greeven,
P. Griffith,
L. Grillo,
S. Gromov,
L. Gruber,
B.R. Gruberg Cazon,
C. Gu,
M. Guarise,
P. A. G{\"u}nther,
E. Gushchin,
A. Guth,
Y. Guz,
T. Gys,
T. Hadavizadeh,
G. Haefeli,
C. Haen,
J. Haimberger,
S.C. Haines,
T. Halewood-leagas,
P.M. Hamilton,
Q. Han,
X. Han,
T.H. Hancock,
S. Hansmann-Menzemer,
N. Harnew,
T. Harrison,
R. Hart,
C. Hasse,
M. Hatch,
J. He,
M. Hecker,
K. Heijhoff,
K. Heinicke,
A.M. Hennequin,
K. Hennessy,
L. Henry,
J. Heuel,
A. Hicheur,
D. Hill,
M. Hilton,
S.E. Hollitt,
P.H. Hopchev,
J. Hu,
J. Hu,
W. Hu,
W. Huang,
X. Huang,
W. Hulsbergen,
R.J. Hunter,
M. Hushchyn,
D. Hutchcroft,
D. Hynds,
P. Ibis,
M. Idzik,
D. Ilin,
P. Ilten,
A. Inglessi,
A. Ishteev,
K. Ivshin,
R. Jacobsson,
S. Jakobsen,
E. Jans,
B.K. Jashal,
A. Jawahery,
V. Jevtic,
M. Jezabek,
F. Jiang,
M. John,
D. Johnson,
C.R. Jones,
T.P. Jones,
B. Jost,
N. Jurik,
S. Kandybei,
Y. Kang,
M. Karacson,
J.M. Kariuki,
N. Kazeev,
M. Kecke,
F. Keizer,
M. Kelsey,
M. Kenzie,
T. Ketel,
B. Khanji,
A. Kharisova,
S. Kholodenko,
K.E. Kim,
T. Kirn,
V.S. Kirsebom,
O. Kitouni,
S. Klaver,
K. Klimaszewski,
S. Koliiev,
A. Kondybayeva,
A. Konoplyannikov,
P. Kopciewicz,
R. Kopecna,
P. Koppenburg,
M. Korolev,
I. Kostiuk,
O. Kot,
S. Kotriakhova,
P. Kravchenko,
L. Kravchuk,
R.D. Krawczyk,
M. Kreps,
F. Kress,
S. Kretzschmar,
P. Krokovny,
W. Krupa,
W. Krzemien,
W. Kucewicz,
M. Kucharczyk,
V. Kudryavtsev,
H.S. Kuindersma,
G.J. Kunde,
T. Kvaratskheliya,
D. Lacarrere,
G. Lafferty,
A. Lai,
A. Lampis,
D. Lancierini,
J.J. Lane,
R. Lane,
G. Lanfranchi,
C. Langenbruch,
J. Langer,
O. Lantwin,
T. Latham,
F. Lazzari,
R. Le Gac,
S.H. Lee,
R. Lef{\`e}vre,
A. Leflat,
S. Legotin,
O. Leroy,
T. Lesiak,
B. Leverington,
H. Li,
L. Li,
P. Li,
X. Li,
Y. Li,
Y. Li,
Z. Li,
X. Liang,
T. Lin,
R. Lindner,
V. Lisovskyi,
R. Litvinov,
G. Liu,
H. Liu,
S. Liu,
X. Liu,
A. Loi,
J. Lomba Castro,
I. Longstaff,
J.H. Lopes,
G. Loustau,
G.H. Lovell,
Y. Lu,
D. Lucchesi,
S. Luchuk,
M. Lucio Martinez,
V. Lukashenko,
Y. Luo,
A. Lupato,
E. Luppi,
O. Lupton,
A. Lusiani,
X. Lyu,
L. Ma,
S. Maccolini,
F. Machefert,
F. Maciuc,
V. Macko,
P. Mackowiak,
S. Maddrell-Mander,
O. Madejczyk,
L.R. Madhan Mohan,
O. Maev,
A. Maevskiy,
D. Maisuzenko,
M.W. Majewski,
S. Malde,
B. Malecki,
A. Malinin,
T. Maltsev,
H. Malygina,
G. Manca,
G. Mancinelli,
R. Manera Escalero,
D. Manuzzi,
D. Marangotto,
J. Maratas,
J.F. Marchand,
U. Marconi,
S. Mariani,
C. Marin Benito,
M. Marinangeli,
P. Marino,
J. Marks,
P.J. Marshall,
G. Martellotti,
L. Martinazzoli,
M. Martinelli,
D. Martinez Santos,
F. Martinez Vidal,
A. Massafferri,
M. Materok,
R. Matev,
A. Mathad,
Z. Mathe,
V. Matiunin,
C. Matteuzzi,
K.R. Mattioli,
A. Mauri,
E. Maurice,
J. Mauricio,
M. Mazurek,
M. McCann,
L. Mcconnell,
T.H. Mcgrath,
A. McNab,
R. McNulty,
J.V. Mead,
B. Meadows,
C. Meaux,
G. Meier,
N. Meinert,
D. Melnychuk,
S. Meloni,
M. Merk,
A. Merli,
L. Meyer Garcia,
M. Mikhasenko,
D.A. Milanes,
E. Millard,
M. Milovanovic,
M.-N. Minard,
L. Minzoni,
S.E. Mitchell,
B. Mitreska,
D.S. Mitzel,
A. M{\"o}dden,
R.A. Mohammed,
R.D. Moise,
T. Momb{\"a}cher,
I.A. Monroy,
S. Monteil,
M. Morandin,
G. Morello,
M.J. Morello,
J. Moron,
A.B. Morris,
A.G. Morris,
R. Mountain,
H. Mu,
F. Muheim,
M. Mukherjee,
M. Mulder,
D. M{\"u}ller,
K. M{\"u}ller,
C.H. Murphy,
D. Murray,
P. Muzzetto,
P. Naik,
T. Nakada,
R. Nandakumar,
T. Nanut,
I. Nasteva,
M. Needham,
I. Neri,
N. Neri,
S. Neubert,
N. Neufeld,
R. Newcombe,
T.D. Nguyen,
C. Nguyen-Mau,
E.M. Niel,
S. Nieswand,
N. Nikitin,
N.S. Nolte,
C. Nunez,
A. Oblakowska-Mucha,
V. Obraztsov,
S. Ogilvy,
D.P. O'Hanlon,
R. Oldeman,
C.J.G. Onderwater,
J. D. Osborn,
A. Ossowska,
J.M. Otalora Goicochea,
T. Ovsiannikova,
P. Owen,
A. Oyanguren,
B. Pagare,
P.R. Pais,
T. Pajero,
A. Palano,
M. Palutan,
Y. Pan,
G. Panshin,
A. Papanestis,
M. Pappagallo,
L.L. Pappalardo,
C. Pappenheimer,
W. Parker,
C. Parkes,
C.J. Parkinson,
B. Passalacqua,
G. Passaleva,
A. Pastore,
M. Patel,
C. Patrignani,
C.J. Pawley,
A. Pearce,
A. Pellegrino,
M. Pepe Altarelli,
S. Perazzini,
D. Pereima,
P. Perret,
K. Petridis,
A. Petrolini,
A. Petrov,
S. Petrucci,
M. Petruzzo,
A. Philippov,
L. Pica,
M. Piccini,
B. Pietrzyk,
G. Pietrzyk,
M. Pili,
D. Pinci,
J. Pinzino,
F. Pisani,
A. Piucci,
Resmi  P.K,
V. Placinta,
S. Playfer,
J. Plews,
M. Plo Casasus,
F. Polci,
M. Poli Lener,
M. Poliakova,
A. Poluektov,
N. Polukhina,
I. Polyakov,
E. Polycarpo,
G.J. Pomery,
S. Ponce,
A. Popov,
D. Popov,
S. Popov,
S. Poslavskii,
K. Prasanth,
L. Promberger,
C. Prouve,
V. Pugatch,
A. Puig Navarro,
H. Pullen,
G. Punzi,
W. Qian,
J. Qin,
R. Quagliani,
B. Quintana,
N.V. Raab,
R.I. Rabadan Trejo,
B. Rachwal,
J.H. Rademacker,
M. Rama,
M. Ramos Pernas,
M.S. Rangel,
F. Ratnikov,
G. Raven,
M. Reboud,
F. Redi,
F. Reiss,
C. Remon Alepuz,
Z. Ren,
V. Renaudin,
R. Ribatti,
S. Ricciardi,
D.S. Richards,
K. Rinnert,
P. Robbe,
A. Robert,
G. Robertson,
A.B. Rodrigues,
E. Rodrigues,
J.A. Rodriguez Lopez,
M. Roehrken,
A. Rollings,
P. Roloff,
V. Romanovskiy,
M. Romero Lamas,
A. Romero Vidal,
J.D. Roth,
M. Rotondo,
M.S. Rudolph,
T. Ruf,
J. Ruiz Vidal,
A. Ryzhikov,
J. Ryzka,
J.J. Saborido Silva,
N. Sagidova,
N. Sahoo,
B. Saitta,
D. Sanchez Gonzalo,
C. Sanchez Gras,
C. Sanchez Mayordomo,
R. Santacesaria,
C. Santamarina Rios,
M. Santimaria,
E. Santovetti,
D. Saranin,
G. Sarpis,
M. Sarpis,
A. Sarti,
C. Satriano,
A. Satta,
M. Saur,
D. Savrina,
H. Sazak,
L.G. Scantlebury Smead,
S. Schael,
M. Schellenberg,
M. Schiller,
H. Schindler,
M. Schmelling,
T. Schmelzer,
B. Schmidt,
O. Schneider,
A. Schopper,
M. Schubiger,
S. Schulte,
M.H. Schune,
R. Schwemmer,
B. Sciascia,
A. Sciubba,
S. Sellam,
A. Semennikov,
M. Senghi Soares,
A. Sergi,
N. Serra,
J. Serrano,
L. Sestini,
A. Seuthe,
P. Seyfert,
D.M. Shangase,
M. Shapkin,
I. Shchemerov,
L. Shchutska,
T. Shears,
L. Shekhtman,
Z. Shen,
V. Shevchenko,
E.B. Shields,
E. Shmanin,
J.D. Shupperd,
B.G. Siddi,
R. Silva Coutinho,
L. Silva de Oliveira,
G. Simi,
S. Simone,
I. Skiba,
N. Skidmore,
T. Skwarnicki,
M.W. Slater,
J.C. Smallwood,
J.G. Smeaton,
A. Smetkina,
E. Smith,
M. Smith,
A. Snoch,
M. Soares,
L. Soares Lavra,
M.D. Sokoloff,
F.J.P. Soler,
A. Solovev,
I. Solovyev,
F.L. Souza De Almeida,
B. Souza De Paula,
B. Spaan,
E. Spadaro Norella,
P. Spradlin,
F. Stagni,
M. Stahl,
S. Stahl,
P. Stefko,
O. Steinkamp,
S. Stemmle,
O. Stenyakin,
H. Stevens,
S. Stone,
M.E. Stramaglia,
M. Straticiuc,
D. Strekalina,
S. Strokov,
F. Suljik,
J. Sun,
L. Sun,
Y. Sun,
P. Svihra,
P.N. Swallow,
K. Swientek,
A. Szabelski,
T. Szumlak,
M. Szymanski,
S. Taneja,
Z. Tang,
T. Tekampe,
F. Teubert,
E. Thomas,
K.A. Thomson,
M.J. Tilley,
V. Tisserand,
S. T'Jampens,
M. Tobin,
S. Tolk,
L. Tomassetti,
D. Torres Machado,
D.Y. Tou,
M. Traill,
M.T. Tran,
E. Trifonova,
C. Trippl,
A. Tsaregorodtsev,
G. Tuci,
A. Tully,
N. Tuning,
A. Ukleja,
D.J. Unverzagt,
A. Usachov,
A. Ustyuzhanin,
U. Uwer,
A. Vagner,
V. Vagnoni,
A. Valassi,
G. Valenti,
N. Valls Canudas,
M. van Beuzekom,
H. Van Hecke,
E. van Herwijnen,
C.B. Van Hulse,
M. van Veghel,
R. Vazquez Gomez,
P. Vazquez Regueiro,
C. V{\'a}zquez Sierra,
S. Vecchi,
J.J. Velthuis,
M. Veltri,
A. Venkateswaran,
M. Veronesi,
M. Vesterinen,
D. Vieira,
M. Vieites Diaz,
H. Viemann,
X. Vilasis-Cardona,
E. Vilella Figueras,
P. Vincent,
G. Vitali,
A. Vitkovskiy,
A. Vollhardt,
D. Vom Bruch,
A. Vorobyev,
V. Vorobyev,
N. Voropaev,
R. Waldi,
J. Walsh,
C. Wang,
J. Wang,
J. Wang,
J. Wang,
J. Wang,
M. Wang,
R. Wang,
Y. Wang,
Z. Wang,
D.R. Ward,
H.M. Wark,
N.K. Watson,
S.G. Weber,
D. Websdale,
C. Weisser,
B.D.C. Westhenry,
D.J. White,
M. Whitehead,
D. Wiedner,
G. Wilkinson,
M. Wilkinson,
I. Williams,
M. Williams,
M.R.J. Williams,
F.F. Wilson,
W. Wislicki,
M. Witek,
L. Witola,
G. Wormser,
S.A. Wotton,
H. Wu,
K. Wyllie,
Z. Xiang,
D. Xiao,
Y. Xie,
H. Xing,
A. Xu,
J. Xu,
L. Xu,
M. Xu,
Q. Xu,
Z. Xu,
Z. Xu,
D. Yang,
Y. Yang,
Z. Yang,
Z. Yang,
Y. Yao,
L.E. Yeomans,
H. Yin,
J. Yu,
X. Yuan,
O. Yushchenko,
K.A. Zarebski,
M. Zavertyaev,
M. Zdybal,
O. Zenaiev,
M. Zeng,
D. Zhang,
L. Zhang,
S. Zhang,
Y. Zhang,
Y. Zhang,
A. Zhelezov,
Y. Zheng,
X. Zhou,
Y. Zhou,
X. Zhu,
V. Zhukov,
J.B. Zonneveld,
S. Zucchelli,
D. Zuliani,
G. Zunica

==> LHCb_authorlist.tex <==
% $Id: LHCb_authorlist.tex 78711 2015-08-06 07:54:32Z apuignav $
% ===============================================================================
% Purpose: example of authorlist for LHCb template
% Author:
% Created on: 2009-09-24
% ===============================================================================

%\documentclass[a4paper]{article}
%\setlength{\oddsidemargin}{0cm}
%\setlength{\evensidemargin}{0cm}
%\setlength{\textwidth}{16.5cm}
%\setlength{\parindent}{0cm}
%\begin{document}
\centerline{\large\normalfont\bfseries LHCb collaboration}
\begin{flushleft}
\small
%-- LHCb Authorlist, Example typesetting
%-- 
A.~N.~Other$^{1}$.\bigskip\newline{\it
\footnotesize
$ ^{1}$University of nowhere\\
}
%-- 
%-- 
\end{flushleft}
%\end{document}


==> Makefile <==
# $Id: Makefile 106572 2017-04-07 10:24:57Z spradlin $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = Xibc2DpK

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 


==> wordcount.tex <==
\ProvidesFile{wordcount.tex}[2000/09/27 v1.5 Michael Downes]
% Copyright 2000 Michael John Downes
% This file has no restrictions on its use, distribution, or sale.
%
% If you run LaTeX on wordcount.tex it will prompt you for the name of a
% document to be counted. For most people, however, it will be more
% convenient to run the shell script wordcount.sh, giving the document
% name as the first argument. The comments in wordcount.sh
% give further information about the usage and limitations of this tool.

% The fundamental idea is to mark each character and interword space
% with a unique tag that will show up in TeX "showbox" output. Then
% arrange to make the output routine trigger a TeX overfull vbox message
% for the page box so that everything gets reported in the TeX log.
% Then run grep -c (or an equivalent text search utility, e.g., perl) on
% the log file to count the occurrences.
%
% In showbox output, a character is typically represented by a line of
% the form
%
%   ...\T1/cmr/m/n/10 e
%
% where "\T1/cmr/m/n/10" is the font name. We arrange things so that all
% characters are typeset in a font named "\3.08632". Furthermore, for
% interword spaces, which are normally represented in the output as
% something like
%
%   ...\glue 3.33333 plus 1.66666 minus 1.11111
%
% we use \spaceskip to ensure that it always appears as
%
%   ...\glue(\spaceskip) 3.08633 plus 9.0
%
% Then to count characters (including word spaces) we can
% grep for lines matching "3.0863", while to count words we
% count the number of lines in the log that match "3.08633" but not
% "3.08632".
%
% For an accurate count in multi-line paragraphs we also need
% to set rightskip to the flag value, since interword spaces are
% discarded at line breaks; and on the presumption that hyphenated
% compounds like "steady-state" should be counted as two words, we set
% \exhyphenpenalty to a value that ensures a line break at *every*
% explicit hyphen---then we will get a rightskip glue node between the
% two parts. (How about em-dashes? you may ask. Answer: it works all
% right, try it and see.)

\ifx\relax\?\def\wcQUIET{TT}\else\def\wcQUIET{TF}\fi

% We want accented letters to be represented by a single font char, to
% the extent possible:
\RequirePackage[T1]{fontenc}
\makeatletter
\thickmuskip=5.55555mu plus5.55555mu minus 2.22222mu
\let\@@thickmuskip\thickmuskip \newmuskip\thickmuskip
\let\@@spaceskip\spaceskip \xspaceskip=0pt
\newskip\@charfontname
% Ensure that these cannot be overridden.
\let\spaceskip\@charfontname \let\xspaceskip\spaceskip
\def\FreezeSpaces{%
  \setbox\z@\hbox{\mathsurround=\z@ $\mkern\@@thickmuskip$}%
  \@@spaceskip=\wd\z@ plus 9pt\relax
  % Setting rightskip to a slightly different value means that
  % end-of-line spaces can be distinguished if desired. (By default,
  % they are not.) Using fil units means there won't be any hyphenation
  % except for explicit hyphens.
  \dimen@\@@spaceskip \advance\dimen@ 1sp\relax
  \rightskip\z@ plus\strip@pt\dimen@ fil\relax
  % Prevent any further changes to \rightskip.
  \let\rightskip\spaceskip
  \@charfontname=\wd\z@ \advance\@charfontname -1sp\relax
  % Cancel all non-1000 sfcodes, which might otherwise affect the value
  % of inter-sentence spaces and keep them from being counted as
  % interword spaces.
  \def\do{\sfcode\fam\@m \advance\fam\@ne
    \ifnum\fam>\@cclv\expandafter\@gobble\fi \do
  }%
  \fam\z@ \do
  \let\frenchspacing\relax \let\nonfrenchspacing\relax
}
\def\DashPatch{%
  \exhyphenpenalty=-\@M \let\exhyphenpenalty\count@
  \hyphenpenalty\@M \let\hyphenpenalty\count@
  % LaTeX bug? Default definitions for these don't have \exhyphenpenalty
  % built in. Change them to just print a hyphen so that the penalties
  % will work.
  \def\textemdash{-}\def\textendash{-}%
}
% Here we set the font to ptmr8t (a T1 encoded font for which most
% people are likely to have a tfm file) and then make it difficult for
% the font to be changed ever again. We use two names for the font,
% \ptmr and \3.08632, the former being easier to use when resetting math
% fonts. The name that is defined last when TeX processes a document is
% the one that will be used in the log file.
\def\FreezeFont{%
  \expandafter\font
    \csname\strip@pt\@charfontname\endcsname
    =ptmr8t \relax
  \ptmr
  \check@mathfonts \let\check@mathfonts\relax
  \def\do{%
    \textfont\fam=\ptmr\scriptfont\fam=\ptmr\scriptscriptfont\fam=\ptmr
    \advance\fam\@ne \ifnum\fam<\sixt@@n \else\expandafter\@gobble\fi
    \do
  }%
  \fam=0 \do
}
\font\ptmr=ptmr8t \relax
\fontdimen22\ptmr=1sp % to permit use as math font 2
\let\selectfont\relax
\let\fontshape\@gobble \let\fontseries\@gobble \let\fontfamily\@gobble 
\let\fontencoding\@gobble \let\fontsize\@gobbletwo
\let\linespread\@gobble 
\let\try@load@fontshape\relax
\@namedef{U/msa/m/n}{}% disable special test in AMS documentclasses
\def\define@newfont{\expandafter\let\font@name=\ptmr}
\let\@@hfuzz\hfuzz \let\@@vfuzz\vfuzz
\newdimen\hfuzz \let\vfuzz\hfuzz
\def\QuietBoxes{%
  \@@hfuzz\maxdimen \@@vfuzz\maxdimen
}
\AtBeginDocument{\FreezeSpaces \FreezeFont \DashPatch \QuietBoxes}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Halign patches
\def\ialign{\everycr{}\tabskip\@@spaceskip\halign} % initialized \halign
\def\extracolsep#1{\tabskip\@@spaceskip}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\nofiles \let\makeindex\@empty % work-around for a natbib problem
% Seize control of the output routine to avoid extra clutter of dvi
% files. Handling \AtBeginDVI would take some extra work--for now I
% won't bother.
\def\showpagebox{%
  \showboxbreadth\maxdimen\showboxdepth99
  % This is a devious way of getting the box contents into the log file
  % without actually using \showbox (which typically results in a
  % nonzero exit code from the TeX run).
  \@@vfuzz\z@
  \setbox\z@\vbox to\z@{\box\@outputbox}%
  \setbox\z@\box\voidb@x
  \global \@colht \textheight
  \stepcounter{page}%
  \let\firstmark\botmark
}
\AtBeginDocument{\def\@outputpage{\showpagebox}}
\if\wcQUIET\else
\begingroup \def\msg^^J#1]^^J{\endgroup\message{#1]^^J^^J}}
\endlinechar=`\^^J \catcode`\ =12 \msg

The 'wordcount' utility provides a way of estimating the number of
words in a LaTeX document.

[Warning: The counting method uses a large log file as an intermediate
step. If your disk space is extremely low the counting process
may end prematurely for lack of space.]

\fi

% \typein has extraneous blank lines and slightly idiosyncratic prompt.
\begingroup \endlinechar=-1
\message{File name [press RETURN to cancel]: }
\def\do{%
  \let\do\@makeother \dospecials
  \global\read-1 to\wcFileName
  \endgroup
}
\do

\ifx\@empty\wcFileName
  \typeout{No file name given; quitting.}\expandafter\@@end\fi

\expandafter\filename@parse\expandafter{\wcFileName}
\edef\jobname{\filename@base}

\if\wcQUIET
  \message{\wcFileName}
\else
\typeout{^^JTo get a count of characters, run^^J^^J \space
%
  grep -c '3[.]0863[23]' wordcount.log^^J^^J%
%
or equivalent when processing is finished.^^J%
}
\fi

\typeout{Processing \wcFileName...^^J}

\IfFileExists{\wcFileName}{\batchmode}{\nonstopmode}
\edef\@tempa{\noexpand\makeatother
  \noexpand\input{\wcFileName}\noexpand\stop
}
\@tempa


==> xibcdecaychannel.tex <==
\appendix
\section*{Appendix}

\begin{sidewaystable}[h]
  \centering
  \caption{Branching ratios for the semi-leptonic decays of \Xibc with charge current.}
  \label{tab:semilepdecay}
  \begin{tabular}{|l r | l r|}
    \toprule
    \multicolumn{1}{|c}{Channels}& \multicolumn{1}{c|}\BF												&
    \multicolumn{1}{c}{Channels}& \multicolumn{1}{c|}\BF \\
    \midrule
    \sigmabmlv			& $1.55\times10^{-3}$		~\cite{Hu:2020mxk}								&
    \xibmlv	 ($\ell=\electron/\muon$)				& $(1.5\pm0.2)\times10^{-2}$		~\cite{Shi:2019hbf}\\
    \sigmabmlv			& $1.12\times10^{-3}$		~\cite{Wang_2017,Gerasimov:2019jwp}				&
    \xibmprlv			& $9.51\times10^{-3}$		~\cite{Hu:2020mxk}\\
    \sigmabmlv ($\ell=\electron/\muon$)				& $(4.2\pm0.7)\times10^{-4}$		~\cite{Shi:2019hbf}	&
    \xibmprlv			& $7.10\times10^{-3}$		~\cite{Wang_2017}\\
    \sigmabmstrlv		& $3.24\times10^{-4}$		~\cite{Hu:2020mxk}								&
    \xibmprlv ($\ell=\electron/\muon$)				& $(1.9\pm0.3)\times10^{-3}$		~\cite{Shi:2019hbf}\\
    \sigmabmstrlv ($\ell=\electron$)					& $3.06\times10^{-4}$			~\cite{Zhao:2018mrg}&
    \xibmprstrlv			& $1.84\times10^{-3}$		~\cite{Hu:2020mxk}\\
    \sigmacplv			& $5.65\times10^{-6}$		~\cite{Hu:2020mxk}								&
    \xibmprstrlv ($\ell=\electron$)					& $1.80\times10^{-3}$			~\cite{Zhao:2018mrg}\\
    \sigmacplv			& $6.52\times10^{-6}$		~\cite{Wang_2017}								&
    \xiccplv			& $6.01\times10^{-3}$		~\cite{Hu:2020mxk,Wang_2017}\\
    \sigmacplv			& $7.00\times10^{-6}$		~\cite{Gerasimov:2019jwp}						&
    \xiccplv			& $6.03\times10^{-3}$		~\cite{Gerasimov:2019jwp}\\
    \sigmacplv ($\ell=\electron/\muon$)				& $(5.9\pm1.0)\times10^{-5}$		~\cite{Shi:2019hbf}	&
    \xiccplv			& $4.6\times10^{-2}$		~\cite{onishchenko2000inclusive}\\
    \sigmacplv ($\ell=\tauon$)						& $(3.5\pm0.5)\times10^{-5}$		~\cite{Shi:2019hbf}	&
    \xiccpstrlv			& $1.49\times10^{-3}$		~\cite{Hu:2020mxk}\\
    \sigmacpstrlv		& $2.51\times10^{-6}$		~\cite{Hu:2020mxk}								&
    \xiccpstrlv ($\ell=\electron$)					& $1.27\times10^{-3}$			~\cite{Zhao:2018mrg}\\
    \sigmacpstrlv ($\ell=\electron$)					& $2.35\times10^{-6}$			~\cite{Zhao:2018mrg}&
    \lcplv				& $2.48\times10^{-6}$		~\cite{Hu:2020mxk}\\
    \xibmlv				& $6.85\times10^{-3}$		~\cite{Hu:2020mxk}								&
    \lcplv				& $2.53\times10^{-6}$		~\cite{Wang_2017}\\
    \xibmlv				& $4.1\times10^{-2}$		~\cite{Berezhnoy:2018bde,onishchenko2000inclusive}	&
    \lcplv				& $3.00\times10^{-6}$		~\cite{Gerasimov:2019jwp}\\
    \xibmlv				& $8.67\times10^{-3}$		~\cite{Wang_2017}								&
    \lcplv ($\ell=\electron/\muon$)					& $(3.1\pm0.7)\times10^{-6}$		~\cite{Shi:2019hbf}\\
    \xibmlv				& $8.68\times10^{-3}$		~\cite{Gerasimov:2019jwp}						&
    \lcplv ($\ell=\tauon$)							& $(1.4\pm0.4)\times10^{-6}$		~\cite{Shi:2019hbf}\\
    \bottomrule
  \end{tabular}
\end{sidewaystable}

\clearpage

\begin{sidewaystable}[h]
  \centering
  \caption{Branching ratios for the non-leptonic decays of \Xibc with \cquark decay.}
  \label{tab:cdecay}
  \begin{tabular}{|l r | l r|}
    \toprule
    \multicolumn{1}{|c}{Channels}& \multicolumn{1}{c|}\BF												&
    \multicolumn{1}{c}{Channels}& \multicolumn{1}{c|}\BF \\
    \midrule
    \sigmabmkp		& $(4.4\pm1.0)\times10^{-5}$		~\cite{Shi:2019hbf}								&
    \xibmprrhop		& $(6.6\pm1.2)\times10^{-3}$		~\cite{Shi:2019hbf}\\
    \sigmabmkp		& $5.99\times10^{-5}$			~\cite{Wang_2017}								&
    \xibmprrhop		& $2.52\times10^{-2}$			~\cite{Wang_2017}\\
    \sigmabmkpstr	& $(6.1\pm1.2)\times10^{-5}$		~\cite{Shi:2019hbf}								&
    \xibmprkp		& $(3.0\pm0.8)\times10^{-4}$		~\cite{Shi:2019hbf}\\
    \sigmabmkpstr	& $1.62\times10^{-4}$			~\cite{Wang_2017}								&
    \xibmprkp		& $4.88\times10^{-4}$			~\cite{Wang_2017}\\
    \sigmabmpip	& $(3.2\pm0.6)\times10^{-4}$		~\cite{Shi:2019hbf}								&
    \xibmprkpstr	& $(2.0\pm0.4)\times10^{-4}$		~\cite{Shi:2019hbf}\\
    \sigmabmpip	& $2.33\times10^{-4}$			~\cite{Gerasimov:2019jwp}						&
    \xibmprkpstr	& $9.90\times10^{-4}$			~\cite{Wang_2017}\\
    \sigmabmpip	& $8.05\times10^{-4}$			~\cite{Wang_2017}								&
    \xibmpip		& $(1.8\pm0.3)\times10^{-2}$		~\cite{Shi:2019hbf}\\
    \sigmabmstrpip	& $1.07\times10^{-4}$			~\cite{Zhao:2018mrg}							&
    \xibmpip		& $7.1\times10^{-2}$			~\cite{Berezhnoy:2018bde}\\
    \sigmabmstrrhop	& $9.09\times10^{-4}$			~\cite{Zhao:2018mrg}							&
    \xibmpip		& $1.23\times10^{-2}$			~\cite{Wang_2017}\\
    \sigmabmstrkp	& $6.53\times10^{-6}$			~\cite{Zhao:2018mrg}							&
    \xibmpip		& $3.53\times10^{-3}$			~\cite{Gerasimov:2019jwp}\\
    \sigmabmstrkpstr	& $4.95\times10^{-5}$			~\cite{Zhao:2018mrg}							&
    \xibmpip		& $7.1\times10^{-2}$			~\cite{onishchenko2000inclusive}\\
    \sigmabmrhop	& $3.06\times10^{-3}$			~\cite{Gerasimov:2019jwp}						&
    \xibmrhop		& $(4.2\pm0.7)\times10^{-2}$		~\cite{Shi:2019hbf}\\
    \sigmabmrhop	& $3.32\times10^{-3}$			~\cite{Wang_2017}								&
    \xibmrhop		& $2.01\times10^{-1}$			~\cite{Berezhnoy:2018bde,onishchenko2000inclusive}\\
    \sigmabmrhop	& $(1.3\pm0.2)\times10^{-3}$		~\cite{Shi:2019hbf}								&
    \xibmrhop		& $2.36\times10^{-2}$			~\cite{Wang_2017}\\
    \sigmabmpitwo	& $2.51\times10^{-3}$			~\cite{Gerasimov:2019jwp}						&
    \xibmrhop		& $2.21\times10^{-2}$			~\cite{Gerasimov:2019jwp}\\
    \sigmabmpithree	& $2.17\times10^{-4}$			~\cite{Gerasimov:2019jwp}						&
    \xibmpitwo		& $1.78\times10^{-2}$			~\cite{Gerasimov:2019jwp}\\
    \sigmabmpifour	& $1.37\times10^{-5}$			~\cite{Gerasimov:2019jwp}						&
    \xibmpithree	& $9.22\times10^{-4}$			~\cite{Gerasimov:2019jwp}\\
    \sigmabmpifive	& $1.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}						&
    \xibmpifour		& $5.52\times10^{-5}$			~\cite{Gerasimov:2019jwp}\\
    \xibmkp		& $1.06\times10^{-3}$			~\cite{Wang_2017}								&
    \xibmpifive		& $1.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}\\
    \xibmkp		& $(1.8\pm0.3)\times10^{-3}$		~\cite{Shi:2019hbf}								&
    \xibmprstrpip	& $1.08\times10^{-3}$			~\cite{Zhao:2018mrg}\\
    \xibmkpstr		& $8.87\times10^{-4}$			~\cite{Wang_2017}								&
    \xibmprstrrhop	& $6.86\times10^{-3}$			~\cite{Zhao:2018mrg}\\
    \xibmkpstr		& $(1.7\pm0.3)\times10^{-3}$		~\cite{Shi:2019hbf}								&
    \xibmprstrkp	& $5.11\times10^{-5}$			~\cite{Zhao:2018mrg}\\
    \xibmprpip		& $(2.2\pm0.4)\times10^{-3}$		~\cite{Shi:2019hbf}								&
    \xibmprstrkpstr	& $2.90\times10^{-4}$			~\cite{Zhao:2018mrg}\\
    \xibmprpip		& $7.11\times10^{-3}$			~\cite{Wang_2017}&&\\    
    \bottomrule
  \end{tabular}
\end{sidewaystable}

\clearpage

\begin{sidewaystable}[h]
  \centering
  \caption{Branching ratios for the non-leptonic decays of \Xibc with \bquark decay.}
  \label{tab:bdecay}
  \begin{tabular}{|l r | l r  | l r|}
    \toprule
    \multicolumn{1}{|c}{Channels}& \multicolumn{1}{c}\BF							&
    \multicolumn{1}{|c}{Channels}& \multicolumn{1}{c}\BF							&
    \multicolumn{1}{|c}{Channels}& \multicolumn{1}{c|}\BF \\
    \midrule
    \sigmacpam		& $(4.9\pm0.7)\times10^{-6}$		~\cite{Shi:2019hbf}			&
    \sigmacpstrkmstr	& $6.84\times10^{-9}$			~\cite{Zhao:2018mrg}		&
    \xiccpstrdmstr	& $2.28\times10^{-5}$			~\cite{Zhao:2018mrg}\\
    \sigmacpam		& $7.3\times10^{-7}$			~\cite{Wang_2017}			&
    \sigmacpstrdm	& $8.05\times10^{-9}$			~\cite{Zhao:2018mrg}		&
    \xiccpstrdms	& $2.29\times10^{-4}$			~\cite{Zhao:2018mrg}\\
    \sigmacpkm		& $(7.9\pm1.4)\times10^{-8}$		~\cite{Shi:2019hbf}			&
    \sigmacpstrdmstr	& $1.20\times10^{-8}$			~\cite{Zhao:2018mrg}		&
    \xiccpstrdmstr	& $5.47\times10^{-4}$			~\cite{Zhao:2018mrg}\\
    \sigmacpkm		& $1.27\times10^{-8}$			~\cite{Wang_2017}			&
    \sigmacpstrdms	& $2.14\times10^{-7}$			~\cite{Zhao:2018mrg}		&
    \xiczdz			& $7\times10^{-7}$				~\cite{Kiselev_2003}\\
    \sigmacpkmstr	& $(1.7\pm0.3)\times10^{-7}$		~\cite{Shi:2019hbf}			&
    \sigmacpstrdmstr& $2.99\times10^{-7}$			~\cite{Zhao:2018mrg}		&
    \lcpam			& $(7.4\pm1.2)\times10^{-7}$		~\cite{Shi:2019hbf}\\
    \sigmacpkmstr	& $2.59\times10^{-8}$			~\cite{Wang_2017}			&
    \xiccppim		& $3.05\times10^{-5}$			~\cite{Gerasimov:2019jwp}	&
    \lcpam			& $6.14\times10^{-7}$			~\cite{Wang_2017}\\
    \sigmacpdm		& $(1.6\pm0.2)\times10^{-7}$		~\cite{Shi:2019hbf}			&
    \xiccppim		& $6.40\times10^{-4}$			~\cite{Wang_2017}			&
    \lcpkm			& $(1.7\pm0.3)\times10^{-8}$		~\cite{Shi:2019hbf}\\
    \sigmacpdm		& $2.72\times10^{-8}$			~\cite{Wang_2017}			&
    \xiccppim		& $0.7\times10^{-2}$			~\cite{onishchenko2000inclusive}&
    \lcpkm			& $1.30\times10^{-8}$			~\cite{Wang_2017}\\
    \sigmacpdmstr	& $(3.6\pm0.5)\times10^{-7}$		~\cite{Shi:2019hbf}			&
    \xiccprhom		& $1.67\times10^{-3}$			~\cite{Gerasimov:2019jwp}	&
    \lcpkmstr		& $(3.0\pm0.5)\times10^{-8}$		~\cite{Shi:2019hbf}\\
    \sigmacpdmstr	& $5.35\times10^{-8}$			~\cite{Wang_2017}			&
    \xiccprhom		& $1.81\times10^{-3}$			~\cite{Wang_2017}			&
    \lcpkmstr		& $2.37\times10^{-8}$			~\cite{Wang_2017}\\
    \sigmacpdms	& $(4.4\pm0.7)\times10^{-6}$		~\cite{Shi:2019hbf}			&
    \xiccprhom		& $1.7\times10^{-2}$			~\cite{onishchenko2000inclusive}& 
    \lcpdm			& $(3.0\pm0.6)\times10^{-8}$		~\cite{Shi:2019hbf}\\
    \sigmacpdms	& $7.40\times10^{-7}$			~\cite{Wang_2017}			&
    \xiccpam		& $2.28\times10^{-3}$			~\cite{Wang_2017}			&
    \lcpdm			& $3.16\times10^{-8}$			~\cite{Wang_2017}\\
    \sigmacpdmsstr	& $(9.1\pm1.4)\times10^{-6}$		~\cite{Shi:2019hbf}			&
    \xiccpkm		& $5.17\times10^{-5}$			~\cite{Wang_2017}			&
    \lcpdmstr		& $(3.7\pm0.6)\times10^{-8}$		~\cite{Shi:2019hbf}\\
    \sigmacpdmsstr	& $1.35\times10^{-6}$			~\cite{Wang_2017}			&
    \xiccpkmstr		& $9.20\times10^{-5}$			~\cite{Wang_2017}			&
    \lcpdmstr		& $3.36\times10^{-8}$			~\cite{Wang_2017}\\
    \sigmacppim	& $(9.8\pm1.8)\times10^{-7}$		~\cite{Shi:2019hbf}			&
    \xiccpdm		& $8.94\times10^{-5}$			~\cite{Wang_2017}			&
    \lcpdms		& $(8.0\pm1.5)\times10^{-7}$		~\cite{Shi:2019hbf}\\
    \sigmacppim	& $1.56\times10^{-7}$			~\cite{Wang_2017}			&
    \xiccpdmstr		& $1.09\times10^{-4}$			~\cite{Wang_2017}			&
    \lcpdms		& $8.65\times10^{-7}$			~\cite{Wang_2017}\\
    \sigmacppim	& $5.00\times10^{-9}$			~\cite{Gerasimov:2019jwp}	&
    \xiccpdms		& $2.37\times10^{-3}$			~\cite{Wang_2017}			&
    \lcpdmsstr		& $(8.9\pm1.6)\times10^{-7}$		~\cite{Shi:2019hbf}\\
    \sigmacprhom	& $(3.2\pm0.5)\times10^{-6}$		~\cite{Shi:2019hbf}			&
    \xiccpdmstr		& $2.57\times10^{-3}$			~\cite{Wang_2017}			&
    \lcpdmsstr		& $8.06\times10^{-7}$			~\cite{Wang_2017}\\
    \sigmacprhom	& $4.91\times10^{-7}$			~\cite{Wang_2017}			&
    \xiccppitwo		& $1.57\times10^{-3}$			~\cite{Gerasimov:2019jwp}	&
    \lcppim		& $(2.1\pm0.3)\times10^{-7}$		~\cite{Shi:2019hbf}\\
    \sigmacprhom	& $4.60\times10^{-7}$			~\cite{Gerasimov:2019jwp}	&
    \xiccppifour		& $1.10\times10^{-3}$			~\cite{Gerasimov:2019jwp}	&
    \lcppim		& $1.57\times10^{-7}$			~\cite{Wang_2017}\\
    \sigmacppitwo	& $5.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}	&
    \xiccppifour		& $1.30\times10^{-3}$			~\cite{Gerasimov:2019jwp}	&
    \lcppim		& $5.10\times10^{-9}$			~\cite{Gerasimov:2019jwp}\\
    \sigmacppithree	& $4.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}	&
    \xiccppifive		& $2.67\times10^{-4}$			~\cite{Gerasimov:2019jwp}	&
    \lcprhom		& $(5.8\pm0.9)\times10^{-7}$		~\cite{Shi:2019hbf}\\
    \sigmacppifive	& $7.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}	&
    \xiccpstrpim		& $1.19\times10^{-4}$			~\cite{Zhao:2018mrg}		&
    \lcprhom		& $4.60\times10^{-7}$			~\cite{Wang_2017}\\
    \sigmacppifive	& $3.10\times10^{-6}$			~\cite{Gerasimov:2019jwp}	&
    \xiccpstrrhom	& $3.13\times10^{-4}$			~\cite{Zhao:2018mrg}		&
    \lcprhom		& $4.30\times10^{-7}$			~\cite{Gerasimov:2019jwp}\\
    \sigmacpstrpim	& $5.79\times10^{-8}$			~\cite{Zhao:2018mrg}		&
    \xiccpstram		& $4.21\times10^{-4}$			~\cite{Zhao:2018mrg}		&
    \lcppithree		& $5.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}\\
    \sigmacpstrrhom	& $1.31\times10^{-7}$			~\cite{Zhao:2018mrg}		&
    \xiccpstrkm		& $9.31\times10^{-6}$			~\cite{Zhao:2018mrg}		&
    \lcppithree		& $4.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}\\
    \sigmacpstram	& $1.86\times10^{-7}$			~\cite{Zhao:2018mrg}		&
    \xiccpstrkmstr	& $1.62\times10^{-5}$			~\cite{Zhao:2018mrg}		&
    \lcppifour		& $4.00\times10^{-7}$			~\cite{Gerasimov:2019jwp}\\
    \sigmacpstrkm	& $4.66\times10^{-9}$			~\cite{Zhao:2018mrg}		&
    \xiccpstrdm		& $9.26\times10^{-6}$			~\cite{Zhao:2018mrg}		&
    \lcppifive		& $1.60\times10^{-6}$			~\cite{Gerasimov:2019jwp}\\
    \bottomrule
  \end{tabular}
\end{sidewaystable}

\clearpage

\begin{sidewaystable}[h]
  \centering
  \caption{Branching ratios for the semi-leptonic decays of \Xibc with FCNC.}
  \label{tab:fcncdecay}
  \begin{tabular}{|l r | l r|}
    \toprule
    \multicolumn{1}{|c}{Channels}& \multicolumn{1}{c|}\BF												&
    \multicolumn{1}{c}{Channels}& \multicolumn{1}{c|}\BF \\
    \midrule
    \sigmaczee		& $2.56\times10^{-9}$			~\cite{Hu:2020mxk}								&
    \xiczmm		& $1.98\times10^{-8}$			~\cite{Xing:2018lre}\\
    \sigmaczee		& $3.78\times10^{-9}$			~\cite{Xing:2018lre}								&
    \xicztt			& $1.22\times10^{-9}$			~\cite{Hu:2020mxk}\\
    \sigmaczmm	& $2.17\times10^{-9}$			~\cite{Hu:2020mxk}								&
    \xicztt			& $4.22\times10^{-9}$			~\cite{Xing:2018lre}\\
    \sigmaczee		& $3.38\times10^{-9}$			~\cite{Xing:2018lre}								&
    \xiczpree		& $4.20\times10^{-8}$			~\cite{Hu:2020mxk}\\
    \sigmacztt		& $1.96\times10^{-10}$			~\cite{Hu:2020mxk}								&
    \xiczpree		& $6.40\times10^{-8}$			~\cite{Xing:2018lre}\\
    \sigmaczee		& $7.16\times10^{-10}$			~\cite{Xing:2018lre}								&
    \xiczprmm		& $3.41\times10^{-8}$			~\cite{Hu:2020mxk}\\
    \sigmaczstree	& $9.92\times10^{-10}$			~\cite{Hu:2020mxk}								&
    \xiczprmm		& $5.59\times10^{-8}$			~\cite{Xing:2018lre}\\
    \sigmaczstrmm	& $8.74\times10^{-10}$			~\cite{Hu:2020mxk}								&
    \xiczprtt		& $2.44\times10^{-9}$			~\cite{Hu:2020mxk}\\
    \sigmaczstrtt	& $1.18\times10^{-10}$			~\cite{Hu:2020mxk}								&
    \xiczprtt		& $9.12\times10^{-9}$			~\cite{Xing:2018lre}\\
    \xiczee			& $1.69\times10^{-8}$			~\cite{Hu:2020mxk}								&
    \xiczprstree		& $1.76\times10^{-8}$			~\cite{Hu:2020mxk}\\
    \xiczee			& $2.06\times10^{-8}$			~\cite{Xing:2018lre}								&
    \xiczprstrmm	& $1.52\times10^{-8}$			~\cite{Hu:2020mxk}\\
    \xiczmm		& $1.59\times10^{-8}$			~\cite{Hu:2020mxk}								&
    \xiczprstrtt		& $1.87\times10^{-9}$			~\cite{Hu:2020mxk}\\ 
    \bottomrule
  \end{tabular}
\end{sidewaystable}
\clearpage


